EgoToM: Benchmarking Theory of Mind Reasoning from Egocentric Videos

We introduce EgoToM, a new video question-answering benchmark that extends Theory-of-Mind (ToM) evaluation to egocentric domains. Using a causal ToM model, we generate multi-choice video QA instances for the Ego4D dataset to benchmark the ability to predict a camera wearer's goals, beliefs, and next actions. We study the performance of both humans and state of the art multimodal large language models (MLLMs) on these three interconnected inference problems. Our evaluation shows that MLLMs achieve close to human-level accuracy on inferring goals from egocentric videos. However, MLLMs (including the largest ones we tested with over 100B parameters) fall short of human performance when inferring the camera wearers' in-the-moment belief states and future actions that are most consistent with the unseen video future. We believe that our results will shape the future design of an important class of egocentric digital assistants which are equipped with a reasonable model of the user's internal mental states.

==> sec/abstract.tex <==
% \begin{abstract}
% Foundation models are becoming increasingly involved in human activities in daily lives through language and other multimodal interactions. When humans interact with others, they attribute intentions and beliefs to observed actions and predict what others will do next. Can multimodal large language models similarly track human behavior in a way that is sensitive to the unobserved internal mental states? We constructed a benchmark to evaluate this ability, referred to as Theory-of-Mind reasoning, using naturalistic human behavior observed in egocentric videos. We use a causal ToM model on specific moments in Ego4D videos to guide QA generation about the camera wearer’s goals, beliefs, and next actions. Our preliminary evaluation suggests that, although multimodal large language models are getting close to human-level accuracy on inferring goals from egocentric videos, they fall short on inferring the camera wearers' in-the-moment belief states and future actions.
% \end{abstract}

\begin{abstract}
We introduce EgoToM, a new video question-answering benchmark that extends Theory-of-Mind (ToM) evaluation to egocentric domains. 
Using a causal ToM model, we generate multi-choice video QA instances for the Ego4D dataset to benchmark the ability to predict a camera wearer’s goals, beliefs, and next actions.
We study the performance of both humans and state of the art multimodal large language models (MLLMs) on these three interconnected inference problems.
Our evaluation shows that MLLMs achieve close to human-level accuracy on inferring goals from egocentric videos. However, MLLMs (including the largest ones we tested with over 100B parameters) fall short of human performance when inferring the camera wearers' in-the-moment belief states and future actions that are most consistent with the unseen video future.
We believe that our results will shape the future design of an important class of egocentric digital assistants which are equipped with a reasonable model of the user's internal mental states.
\footnote{The benchmark will be shared with release of the paper.}

% old abstract
% We introduce EgoToM, a new video question-answering benchmark that extends Theory-of-Mind evaluation to egocentric domains. Using a causal ToM model, we generate multi-choice video QA instances for the Ego4D dataset to benchmark multimodal large language models (MLLMs)’ ability to predict a camera wearer’s goals, beliefs, and next actions. We study the performance of both humans and state of the art MLLMs on these three interconnected inference problems. Our evaluation shows that MLLMs achieve close to human-level accuracy on inferring goals from egocentric videos. However, MLLMs (including the largest ones we tested with over 100B parameters) fall short of human performance when inferring the camera wearers’ in-the-moment belief states and future actions. We believe that our results will shape the future design of an important class of egocentric digital assistants which are equipped with a
% reasonable model of the user’s internal mental states. 
% \footnote{Code for running the benchmark will be published with release of the paper.}
\end{abstract}
